CausalDriveBench: Evaluating Causal Reasoning in Vision-Language-Action Models for Autonomous Driving

Vision-Language-Action (VLA) models for autonomous driving produce natural-language reasoning alongside predicted trajectories, but whether this reasoning reflects the causal structure of the scene remains untested. We introduce CausalDriveBench, an evaluation framework grounded in Pearl's Causal Hierarchy (PCH) that tests causal reasoning in driving-specific VLAs through structured visual question answering (QA) and alternative-trajectory prediction. To this end, we construct causal scene graphs over nuScenes that distinguish causally active, dormant, and distractor entities, separating perceptual salience from causal relevance. The benchmark spans all four rungs of PCH (association, intervention, and counterfactual along with causal discovery) for QA generation. For the higher rungs, we additionally provide reference trajectories under specified scene modifications, enabling action-level verification that complements reasoning-level evaluation. In total, the benchmark contains 7,285 verified causal QA pairs and 1,000 counterfactual trajectories derived from nuScenes. We evaluate 10 driving-specific VLAs and 3 general-purpose VLMs, and report three findings. First, the best model reaches only 70.6% QA accuracy, and 4 of 13 models score below random chance. Second, comparing each driving VLA to the general-purpose VLM that shares its language backbone, the cost of driving fine-tuning ranges from 2 to 34 percentage points on causal QA, with post-training design explaining the spread. Third, causal QA and trajectory accuracy are statistically uncorrelated across models: under counterfactual prompts, predicted trajectories either over-react or collapse onto the observed-scene baseline. Taken together, these results show that neither fluent rationales nor accurate observed-scene trajectories constitute evidence of causal understanding.

==> Styles/causaldrivebench/benchmark_construction_pipeline.tex <==
\subsection{Benchmark Construction Pipeline}
\label{subsec:pipeline}

% [trimed version]
% The benchmark is constructed in four stages (Fig.~\cref{fig:pipeline}):
% (1) causal scene graph extraction, (2) subgraph enumeration and diversity sampling,
% (3) question–answer generation, and (4) counterfactual trajectory synthesis.
The benchmark is constructed in five stages including a preprocessing stage, illustrated in \cref{fig:pipeline}. (0) Preprocessing and input generation (1) Causal scene graph extraction, (2) Subgraph enumeration and diversity sampling, (3) Question–answer generation, and (4) Counterfactual trajectory synthesis.


% Stage~0 assembles the multimodal scene representation from nuScenes ground truth data. Stage~1 extracts a causal scene graph from sensor data; Stage~2 selects a diverse subset via hierarchical clustering and enumerates causal subgraphs; Stage~3 generates question-answer pairs over the selected graphs; Stage~4 synthesises ground-truth counterfactual trajectories for a budgeted subset of binary questions.

\paragraph{Stage 0: Preprocessing and Inputs generation.} 2D bounding boxes for visual entities are projected and rendered onto camera frames with entity labels, the HD map is rasterised and overlaid with ego and agent footprints to produce a top-down BEV, and ego pose plus per-frame annotations are compiled into a structured state record (navigation command, ego kinematics, and per-agent positions). The four-camera stack and BEV are produced for each of four timesteps spanning $[t_0 - 1.5\text{s},\, t_0]$ at 2Hz.

\paragraph{Stage 1: Causal scene graph extraction.}

% [trimed version]
For each scene, we extract a causal scene graph in a single pass using
Claude Opus~4.7~\citep{}, conditioned on multi-view images, BEV frames,
and agent state (position, speed, heading) over a 1.5\,s window.
The prompt uses structured decision trees to infer entities, ego edges,
causal status, and inter-node relations. Full details are provided in ~\cref{app:causal_schema}.

% For each scene, we extract a causal scene graph in a single pass using Claude Opus~4.7~\citep{}, conditioned on multi-view camera images (front, front-left, front-right, back), BEV frames at four timesteps spanning $[t_0 - 1.5\text{\,s}, t_0]$, four BEV frames at the same timesteps, and a filtered \texttt{state.json} file containing position, speed, heading, and lane assignment for ego and all referenced agents. The extraction prompt is structured as a sequence of binary decision trees covering scene inventory, lane classification, ego-state inference, ego-edge assignment, causal-status determination, and inter-node edge construction. Full prompt structure and decision-tree details are in
% Appendix~\cref{app:pipeline}.

\paragraph{Stage 2: Subgraph enumeration and diversity sampling.}

% [trimed version]
We deterministically extract canonical causal subgraphs
(direct, chain, collider, confounding) using fixed priority rules
and generate per-scene subgraph manifests for QA generation.
To select a diverse subset, scenes are hierarchically clustered
by causal structure (L1) and scene context (L2),
retaining one high-richness representative per L2 cluster.
Details are in \cref{app:subgraph_enumeration,app:clustering}.

% We extract canonical causal substructures
% (direct, chain, collider, observed and unobserved confounding)
% from each scene graph through a deterministic procedure
% that resolves overlaps via fixed priority rules
% (confounding subsumes collider at the pair level;
% pure chains require distal nodes that are not themselves ego parents).
% The output is a per-scene subgraph manifest
% with stable structure identifiers consumed by the QA prompts.
% To select a diverse benchmark subset,
% we cluster scenes hierarchically over two complementary kernel families:
% an L1 kernel over causal structure
% (active edges, dormant edges, distractors, subgraph topology)
% and an L2 kernel over scene context
% (road geometry, environment, navigation intent, ego behaviour).
% Within each second-level group
% we retain the highest-richness leader at a sampling rate of 0.5.
% Kernel definitions, weights,
% and the Kneedle threshold selection
% are detailed in Appendix~\cref{app:pipeline}.

\paragraph{Stage 3: Question-answer generation.}

% [trimed version]
QA pairs are generated using three role-specific prompts
targeting active, dormant, and distractor entities.
These prompts instantiate CaLM scenarios for active elements
and specialized discrimination queries for dormant and 
counterfactual queries for distractor elements.
All prompts enforce graph grounding,
perspective consistency, and vocabulary control. More details can be found 
in the \cref{app:qa_generation}

% QA pairs are generated by three role-specific prompts
% that operate over the same scene graph
% but target disjoint entity sets:
% an active-element prompt enumerating all four graph structures
% and instantiating twelve CaLM causal scenarios across PCH layers
% (Table~\cref{tab:active-types});
% a dormant-element prompt classifying each dormant entity
% by activation plausibility, latency mechanism,
% and trajectory sensitivity before generating DQ, EL, and AB questions;
% and a distractor-element prompt classifying each distractor
% by visual salience and counterfactual coherence
% before generating CI, NI, WC, and DR-Empty questions.
% All three prompts share four discipline rules:
% a mandatory scratchpad forcing explicit graph parsing
% before question writing,
% a restricted scene-level preamble with per-question
% \texttt{spatial\_context} for geometry-grounded questions,
% second-person questions and first-person answers
% to prevent voice leakage,
% and a banned-word list excluding graph terminology
% and pipeline labels from all surface text.

\paragraph{Stage 4: Counterfactual trajectory generation.}

% [trimed version]
For each scene, we synthesize ground-truth counterfactual trajectories
for at most one Rung~2 and one Rung~3 binary question.
Trajectory generation prioritizes behavior-changing,
scene-specific interventions.
Synthesis uses LLM-based state mutation of agents followed by
tool-grounded waypoint planning with collision and kinematic checks.
Full implementation details are in \cref{app:counterfactual_traj}.

% For every scene we generate ground-truth alternate ego trajectories
% under at most one Rung~2 binary intervention
% and at most one Rung~3 binary counterfactual,
% drawn from the trajectory-eligible question types.
% The per-scene budget allocates trajectory synthesis
% to questions that maximise three preferences in order:
% trajectory-changing answers over no-change answers,
% scene-specific over policy-level reasoning,
% and unique behavioural effects over redundant ones.
% Synthesis proceeds in three sub-stages:
% (4a) a Claude Haiku~4.5 judge re-evaluates
% the QA generator's \texttt{trajectory\_changes} flag
% and infers auxiliary agent pins;
% (4b) Claude Opus~4.6 mutates entity states
% for non-deterministic actions
% (\texttt{state\_change}, \texttt{reposition},
% \texttt{speed\_change}, \texttt{activate});
% (4c) a tool-using agent (Claude Opus~4.7)
% commits waypoints one at a time
% against a tool surface exposing lane centerlines,
% post-intervention agents, and road features,
% with deterministic in-loop checks for lane-snap,
% collision (SAT polygon overlap),
% and kinematic feasibility.
% A deterministic post-process re-integrates the committed waypoints
% into a smoothed trajectory whose physical consistency
% is guaranteed by construction.
% Full tool surface specification,
% kinematic bounds, and the post-process formulation
% are in Appendix~\cref{app:pipeline}.

==> Styles/causaldrivebench/causal_scene_graph.tex <==
\subsection{Causal Scene Graph}
\label{subsec:causal_graph}

All benchmark labels such as the causal-status annotations, QA pairs, and counterfactual trajectories are derived from the \emph{causal scene graph}, which defines entities in the scene, their causal relations to ego, and inter-dependencies.

\subsubsection{Schema}
\label{subsubsec:schema}

% [trimmed version]-gayatri
% For each scene, the causal scene graph is a directed graph
% $\mathcal{G} = (\mathcal{V}, \mathcal{E}_{\text{ego}}, \mathcal{E}_{\text{inter}})$
% encoding causal relations between scene entities and the ego vehicle,
% with an auxiliary distractor set $\mathcal{D}$ retained for evaluation.
For each driving scene, the causal scene graph is a directed graph
$\mathcal{G} = (\mathcal{V}, \mathcal{E}_{\text{ego}}, \mathcal{E}_{\text{inter}})$
encoding the causal relationships between visually grounded scene entities
and the ego vehicle, together with an auxiliary set $\mathcal{D}$
of causally irrelevant distractors retained for evaluation.

% [trimmed version]-gayatri
% Nodes $\mathcal{V}$ fall into four mutually exclusive types
% (\texttt{EGO}, \texttt{OTHER\_AGENT}, \texttt{TRAFFIC\_CONTROL},
% \texttt{ROAD\_OBSTACLE}) derived from a decision tree over agency
% and rule imposition (Appendix~\ref{app:schema}).

Nodes $\mathcal{V}$ fall into four mutually exclusive types - \texttt{EGO}, \texttt{OTHER\_AGENT}, \texttt{TRAFFIC\_CONTROL}, and \texttt{ROAD\_OBSTACLE} - derived from a binary decision tree over agency and rule imposition (\cref{app:graph_schema}). Each node records standard spatial position, visibility in cameras, lane assignment, and motion attributes.

% [trimmed version]-gayatri
% Ego edges $\mathcal{E}_{\text{ego}}$ take one of four effect types
% (grant, inhibit, longitudinal constraint, lateral constraint)
% and carry a causal status
% $\text{cs}(e) \in \{\texttt{active-sustaining},
% \texttt{active-triggering}, \texttt{dormant}\}$.
Ego edges $\mathcal{E}_{\text{ego}} \subseteq \mathcal{V} \times \{\text{ego}\}$ take one of four effect types - \texttt{GRANTS\_PROCEED}, \texttt{INHIBITS\_PROCEED}, \texttt{CONSTRAINS\_LONGITUDINAL}, \texttt{CONSTRAINS\_LATERAL} - derived from a parallel decision tree over discrete-vs-continuous control and axis-or-polarity (\cref{app:graph_schema}). Each edge also records a causal status, formalized in \cref{subsubsec:causal_status}.

% [trimmed version]-gayatri
% Inter-node edges encode observed causal influence (\texttt{AFFECTS})
% and unobserved common causes (\texttt{CONFOUNDED\_BY}),
% forming a semi-Markovian ADMG with explicit latent confounding.
Inter-node edges $\mathcal{E}_{\text{inter}}$ encode dependencies between non-ego entities, with two relations: directed \texttt{AFFECTS} for observable causal influence and bidirected \texttt{CONFOUNDED\_BY} for unobserved common causes.
This combination of edges makes $\mathcal{G}$ a semi-Markovian acyclic
directed mixed graph (ADMG), allowing unobserved common causes
to be explicitly represented rather than assumed away.

\subsubsection{Causal Status: Active, Dormant, and Distractor}
\label{subsubsec:causal_status}

% [trimmed version]-gayatri
CausalDriveBench distinguishes entities that currently affect ego behavior, could affect it under minimal scene change, or are merely visible, grounded in Pearl’s interventional semantics \citep{pearl2009causal}. Every ego edge encodes the claim that removing the source entity - formally, applying the intervention $\text{do}(X = \text{absent})$ - would alter ego's behavior. The three-way partition follows from how this claim is evaluated.

\paragraph{Active edges.}

% [trimmed version]-gayatri
% An ego edge is \emph{active} if removing the entity over
% the observation window changes ego’s state at $t_0$.
An ego edge is \emph{active} if removing the entity $X$ from the observation window $[t_0 - \Delta, t_0]$ would change ego's state at $t_0$:

\begin{equation}
    \text{active}(e) \iff
    S(\mathcal{G}_{t_0}) \neq S\!\left(\mathcal{G}_{t_0}^{-X}\right),
    \label{eq:active}
\end{equation}

% [trimmed version]-gayatri
% where $S=(s,a,h)$ is ego state and $\Delta=1.5$s matches the BEV horizon.

% [trimmed version]-gayatri
% Active edges are labeled sustaining or triggering,
% affecting downstream counterfactual framing.

where $S(\cdot) = (s, a, h)$ is ego's state vector (speed, acceleration class, heading change), $\mathcal{G}_{t_0}^{-X}$ denotes the counterfactual graph in which $X$ has been absent throughout the window, and $\Delta = 1.5$\,s is the observation window. Active edges are further sub-classified as \emph{sustaining} (a live constraint at $t_0$) or \emph{triggering} (committed earlier in the window but no longer binding at $t_0$); the distinction does not affect graph inclusion but determines the temporal framing of downstream counterfactual questions (see \cref{app:causal_graph} for more details).

\paragraph{Dormant edges.}

% [trimmed version]-gayatri
% An ego edge is \emph{dormant} if it is currently inactive,
% but could become active via a single physically realizable transition
% within $\delta=0.5$s.
An ego edge is \emph{dormant} if it currently inactive, but could become active via a single physically realizable transition within one decision horizon $\delta = 0.5$\,s:
\begin{equation}
    \text{dormant}(e) \iff
    \neg\,\text{active}(e) \,\wedge\,
    \exists\, x' \in R_\delta(X)
    \text{ s.t. } \text{active}(e \mid X \mapsto x'),
    \label{eq:dormant}
\end{equation}

% [trimmed version]-gayatri
% The $\delta$-bound enforces a finite, physically grounded reachability test;
% detailed constraints are given in Appendix~\ref{app:causal-status}.
The $\delta$-bound replaces the unbounded existential over ``plausible modifications'' with a temporally finite, physically grounded single-step reachability test. We restrict $R_\delta(X)$ to transitions arising from the entity's own agency and impose three geometric conditions (single-step reachability, no physical barrier, spatial relevance); see \cref{app:causal_graph} for the full operational restriction.

\paragraph{Distractors.}

% [trimmed version]-gayatri
% A visible entity is a \emph{distractor} if none of its ego edges
% are active or dormant.
A visible entity $X$ is a \emph{distractor} if it's ego edge $(X, \text{ego})$ is neither active nor dormant:
\begin{equation}
    \text{distractor}(X) \iff
    \forall\, e = (X, \text{ego}) :
    \neg\,\text{active}(e) \,\wedge\,
    \neg\,\text{dormant}(e),
    \label{eq:distractor}
\end{equation}

% [trimmed version]-gayatri
% Distractors are excluded from ego edges and retained for
% rejection-style questions probing causal irrelevance.
Distractors are excluded from $\mathcal{E}_{\text{ego}}$ and recorded in $\mathcal{D}$ with a rejection reason grounded in observable scene geometry. Overall, this partition is exhaustive: active entities support all PCH layers, dormant entities support queries up to Rung~2, and distractors support rejection queries across Rungs~1--3.


==> Styles/causaldrivebench/quality_control_and_validation.tex <==
\subsection{Quality Control and Validation}
\label{subsec:quality_control}

% Because all benchmark labels are generated through an LLM-assisted pipeline,
% systematic validation is required at the graph level
% before downstream QA generation,
% and at the QA level before the benchmark is released.
% We apply three passes to the 3{,}189 verified samples
% emerging from Stage~1,
% followed by independent audits of the QA pairs
% and counterfactual trajectories.


% The 3{,}189 samples were allocated across seven annotators,
% each responsible for a contiguous block of roughly 100--140 scenes.
% Reviewers operated through a custom annotation tool
% displaying the four-camera stack,
% the BEV,
% the filtered \texttt{state.json},
% and the extracted graph side by side,
% and could accept, flag for further review,
% or directly edit each sample.
% Approximately 46\% of samples received reviewer edits,
% with recurring patterns falling into four categories:
% edge re-classification,
% causal-status correction,
% edge addition and removal,
% and inter-node edge correction.
% Inter-reviewer agreement on a 5\% double-annotated subset
% reached $\kappa = [\cdot]$ for node classification
% and $\kappa = [\cdot]$ for edge causal status.
% Patterns that recurred consistently enough across reviewers
% were promoted to a deterministic post-processor
% enforcing six structural invariants
% (e.g., dropping indirect-control inter-node edges,
% demoting behind-ego agents to distractors,
% reverse-reachability pruning);
% rule definitions are in Appendix~\ref{app:quality}.
% A final language-model alignment pass
% re-aligns the free-text scene-context fields
% with the corrected graph structure,
% ensuring that downstream QA generation
% conditions on prose consistent with the post-processed graph.


% We manually verified a stratified random sample
% of 702 QA pairs (9.6\% of the benchmark),
% combining a per-type floor of 30 questions
% with a 2\% proportional top-up
% on the highest-volume types.
% A single annotator rated each question
% on three criteria:
% well-formedness,
% answer correctness under the post-processed graph,
% and reasoning consistency.
% Across the audit,
% $[X]\%$ of QA pairs were rated valid,
% yielding a Wilson-score 95\% confidence interval
% of $[\cdot, \cdot]$.
% Per-type validity rates
% and dominant failure modes
% are reported in Appendix~\ref{app:quality}.


% Every synthesised counterfactual trajectory
% is independently re-checked by an offline audit script.
% For each waypoint
% the auditor recomputes ego-versus-agent
% SAT polygon overlap
% against every active agent at its anchor pose,
% and drivable-area membership
% against the nuScenes \texttt{drivable\_area} layer
% in the global frame.
% A trajectory is admitted as ground truth
% iff no waypoint raises either flag;
% failing trajectories are eliminated
% and the parent question is excluded
% from the trajectory-evaluation subset
% (the QA pair itself remains in the QA evaluation,
% since its categorical answer
% does not depend on the trajectory).
% The audit eliminated $[N]\%$ of synthesised trajectories,
% leaving $[M]$ verified counterfactual trajectories
% that serve as ground-truth labels
% for the CF-ADE metric of \S\ref{sec:experiments}.

Since all labels are generated via an LLM-assisted pipeline,
we apply systematic validation at the graph extraction, QA,
and counterfactual-trajectory generation levels.
Seven annotators reviewed the 3{,}189 samples using a custom tool
displaying camera views, BEV, agent state, and extracted graphs.
Reviewers could accept or edit samples; 46\% required edits, primarily correcting edges and causal status. Recurring issues were formalized into deterministic post-processing rules fixes. Final alignment ensures consistency between prose and graph structure. Independent human verification of a stratified 5\% random sample ($n = 365$ of $7{,}285$) found an observed error rate of $\hat{p} = 0.82$\%  (95\% Wilson CI: $[0.28, 2.39]$\%), statistically rejecting the hypothesis that CausalDriveBench's error rate exceeds 5\% at $p = 0.000125$ (one-sided $z$-test, $z = -3.66$), confirming the benchmark-quality fidelity of our iterative VLM-assisted question generation and review pipeline. Additionally, all synthesized counterfactual trajectories are audited for collisions and drivable-area violations eliminating 117 of the synthesized trajectories leaving 1000 verified counterfactual trajectories. See \cref{app:examples} for annotation pipeline and scene examples.


==> Styles/causaldrivebench/question_type_taxonomy.tex <==
\subsection{Question Type Taxonomy}
\label{subsec:qa_taxonomy}

% [trimmed version]
% CausalDriveBench organizes question types by causal status
% (\emph{active}, \emph{dormant}, \emph{distractor}),
% with each family targeting distinct levels of Pearl’s Causal Hierarchy,
% summarized in Tables~\ref{tab:question_taxonomy},
% \ref{tab:dormant_taxonomy}, and \ref{tab:distractor_taxonomy}.

% [trimmed version]
% The \emph{active} taxonomy follows CaLM~\cite{chen2024causal},
% which structures causal evaluation by ladder rung, scenario,
% and domain. Active questions instantiate standard causal scenarios
% (e.g., CaI, CDE, SC, NC, CoI) grounded in scene graph structure.
% Dormant and distractor questions extend CaLM to causally inactive
% but visible entities (e.g., DQ, AB, NI, WC),
% which text-only benchmarks cannot assess.
% See Appendix~\ref{sec:active_qa} for full details.

CausalDriveBench organizes question types by the causal status of the target element: \emph{active}, \emph{dormant} or \emph{distractor}. Each family targets a distinct range of Pearl's Causal Hierarchy, summarized in Tables~\ref{tab:question_taxonomy}. Our taxonomy for causally \emph{active} nodes is grounded in the CaLM framework~\cite{chen2024causal}, which structures causal evaluation as a product of \emph{causal ladder} (rung), \emph{causal scenario} (the specific reasoning task), and \emph{domain}. Active question types instantiate established causal scenarios such as Causal Identification (CaI), Controlled Direct Effect (CDE), Sufficiency Cause (SC), Necessity Cause (NC), Confounder Identification (CoI), grounded in scene graph structure \cref{tab:active_graph_map}. Dormant and distractor types extend the CaLM  to reasoning about causally dormant or causally irrelevant but visible entities such as Dormancy Discrimination (DQ), Activation Boundary (AB), Null Intervention (NI), Wild Counterfactual (WC) and others. See \cref{app:qa_taxonomy} for full details.

==> Styles/causaldrivebench/task_definition.tex <==
\subsection{Task Definition}
\label{subsec:task_def}







%CausalDriveBench evaluates two complementary capabilities of a driving VLA:whether it can recover the \emph{causal structure} of a scene,and whether that understanding translates into appropriate trajectory changesunder hypothetical scene modifications.The benchmark provides multi-view camera images, a navigation command,and a structured query, and requires a reasoned answer and,when applicable, an ego trajectory.

%%Given a scene and a question from the taxonomy in \S\ref{qa_type},the model predicts a categorical answer with reasoning.Questions include binary and four-option multiple-choice formatsspanning causal discovery and all three rungs of PCH,together with novel types targeting dormant and distractor entities.We report accuracy by question type and rung,and use an LLM-as-judge to evaluate reasoning quality.

%\paragraph{Counterfactual trajectory prediction.}Given a counterfactual premise defined as a structured modificationto the causal scene graph (\S\ref{csg}),the model generates an alternative ego trajectory.We measure ADE against ground-truth counterfactual trajectoriesto test whether causal reasoning affects behavior at the action level.

%Success on CausalDriveBench requires more than perceptual descriptionor trajectory regression:a model must identify causally active entities,distinguish them from salient but irrelevant ones,reason under interventions and counterfactuals,and reflect this reasoning in its planned trajectory.


CausalDriveBench evaluates two complementary capabilities of a driving VLA: whether it can recover the \emph{causal structure} of a scene, and whether that causal understanding translates into corresponding changes in planned trajectory under hypothetical scene modifications. The benchmark presents a model with multi-view camera images (front, front-left, front-right, rear), a navigation command, and a structured query, and asks it to produce an answer with reasoning and, for planning tasks, an ego trajectory. \textbf{Causal QA:} Questions are either binary or multiple-choice with four options, spanning causal discovery and all three rungs of PCH, together with seven novel types for dormant and distractor elements that probe the boundary between perceptual salience and causal relevance (see \cref{subsec:qa_taxonomy}). We report accuracy per question type and per rung, and apply LLM-as-judge to evaluate reasoning quality. \textbf{Counterfactual trajectory prediction:} Given a scene and a counterfactual premise, the model must produce an alternative ego trajectory consistent with the altered causal structure. We measure ADE against the ground-truth counterfactual trajectories, to test whether causal reasoning affects behavior at the action level.

Success on CausalDriveBench therefore requires more than perceptual description or trajectory regression: a model must identify which entities cause ego's current behaviour, distinguish them from visually salient but causally inert entities, reason about how behaviour would change under interventions and counterfactuals, and reflect that reasoning in its planned trajectory.
